Synthetic Multimodal Dataset for Empowering Safety and Well-being in Home Environments

This paper presents a synthetic multimodal dataset of daily activities that fuses video data from a 3D virtual space simulator with knowledge graphs depicting the spatiotemporal context of the activities. The dataset is developed for the Knowledge Graph Reasoning Challenge for Social Issues (KGRC4SI), which focuses on identifying and addressing hazardous situations in the home environment. The dataset is available to the public as a valuable resource for researchers and practitioners developing innovative solutions recognizing human behaviors to enhance safety and well-being in

==> ScriptEditor.tex <==
\begin{figure*}[ht]
\centering
%\includegraphics[width=1.0\linewidth]{fig/supportTool.eps}
  \caption{データ作成支援ツールの画面例}\label{Fig2}
\end{figure*}

The VirtualHome currently used for data generation, to which we have added our motions, has about 30 motions that the character can perform and seven kinds of Western-style one-story houses.
Each house has about 400 objects, such as furniture, but not all can be held, carried, or used for motion. Also, due to the limitation of the character's movement by VirtualHome, for example, the character may sit on a chair in an undesirable position or direction, which is unnatural.
Therefore, when creating data, it is necessary to select and combine the movements that can be performed by VirtualHome and the objects that can be used as targets and check the created data for unnatural behaviors. 
The tool described here is designed to support this series of data creation.
%現在データ生成に用いているVirtualHomeは我々が独自にモーションを追加しているものであり, キャラクタが実行できる動作が約30種類, 家屋が洋風の平屋7種類である.
%それぞれの家屋には約400種類の家具などのオブジェクトが配置されているが, すべてのオブジェクトを持ったり, 
%運んだり動作の対象にできるわけではない. またVirtualHomeによるキャラクタの動作の限界から, 
%例えば、椅子に座る場合でも望ましくない位置や向きに座るなどの不自然な動作をすることがある.
%そのためデータを作成する場合には, VirtualHomeで実行できる動作と対象にできるオブジェクトを選んで組み合わせ,
%作成されたデータを不自然な動作をしていないかどうか確認する必要がある. ここで説明するツールは
%この一連のデータ作成を支援するものである.

Figure\ref{Fig2} is an example of the screen of the data creation support tool.
It consists of the following four major parts.
%図\ref{Fig2}は, データ作成支援ツールの画面例である.
%大きく次の4つのパーツから構成されている.
\begin{itemize}
\item In the left window, SPARQL is used to search for existing knowledge graphs to use as reference information for newly created scripts. By default, given the script's name, SPARQL displays the actions described in the script and the objects to which the actions are applied.

\item In the central window, you can select the actions your character can perform and the objects that can perform those actions and create a sequence for your character. Objects can be selected from VirtualHome by using the API to retrieve objects already placed in the specified house and from which the character can perform the actions. Since the Home Object Ontology and the Primitive Action Ontology are used to convert between Japanese and English, the operator can create a sequence of actions in Japanese.

\item In the right window, the character action sequences created in the center window are converted into a script used as an input script for VirtualHome. The script is edited in this window to create a movie and a knowledge graph. 

\item The created video is displayed in the window below, and the user can check if the created video is not unnatural or not.
%\item 左の窓は, 新しく作成する台本の参考情報として利用するために, 既存のナレッジグラフに対してSPARQLで検索を行い, デフォルトで, 台本の名前を指定すると, 台本に記述された動作と動作対象のオブジェクトが表示されるSPARQLが提供されている.
%\item 中央の窓では, キャラクタが実行できる動作とその動作を行うことができる対象物を選択し, キャラクタの動作列を作成する. 対象物はVirtualHomeからAPIを用いて、指定された家屋に配置済みの物体を取り出し、そこから動作の対象にすることが可能なものを選択できる. Home Object OntologyとPrimitive Action Ontologyを用いて日本語と英語の間の変換を行うため, 作業者は日本語で動作列を作成することができる.
%\item 右側の窓には, 中央の窓で作成されたキャラクタの動作列を, VirtualHomeの入力スクリプトになる台本に変換し, 表示する. この窓で台本を編集し, 動画とナレッジグラフを作成する. 
%\item 作成された動画は, 下の窓に表示され, 利用者は作成された動画が不自然なものでないかどうか確認することができる.
\end{itemize}
